mGPT: Few-Shot Learners Go Multilingual

Recent studies report that autoregressive language models can successfully solve many NLP tasks via zero- and few-shot learning paradigms, which opens up new possibilities for using the pre-trained language models. This paper introduces two autoregressive GPT-like models with 1.3 billion and 13 billion parameters trained on 60 languages from 25 language families using Wikipedia and Colossal Clean Crawled Corpus. We reproduce the GPT-3 architecture using GPT-2 sources and the sparse attention mechanism; Deepspeed and Megatron frameworks allow us to parallelize the training and inference steps effectively. The resulting models show performance on par with the recently released XGLM models by Facebook, covering more languages and enhancing NLP possibilities for low resource languages of CIS countries and Russian small nations. We detail the motivation for the choices of the architecture design, thoroughly describe the data preparation pipeline, and train five small versions of the model to choose the most optimal multilingual tokenization strategy. We measure the model perplexity in all covered languages and evaluate it on the wide spectre of multilingual tasks, including classification, generative, sequence labeling and knowledge probing. The models were evaluated with the zero-shot and few-shot methods. Furthermore, we compared the classification tasks with the state-of-the-art multilingual model XGLM. source code and the mGPT XL model are publicly released.

==> tables/generation.tex <==
\begin{table*}[th!]
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{llll}
\toprule

\textbf{ISO} & \textbf{Prompt}                                                                  & \textbf{Result}     &  \\ \midrule
en                                      & The guests hid behind the sofa holding the cake because                 & \cellcolor[HTML]{FFFFFF}\textit{because they were afraid of the cold.}                            &  \\
ua                                      &\begin{ukrainian}Гості сховалися за диваном, тримаючи торт, бо\end{ukrainian}                          & \cellcolor[HTML]{FFFFFF}\begin{ukrainian}бо він був випечений на місці.\end{ukrainian}                                             &  \\
                                        &                                                                                  & \textit{because it was baked on the spot.}                                                         &  \\
fr                                      & Les invités se sont cachés derrière le canapé tenant le gâteau parce que & \cellcolor[HTML]{FFFFFF}parce que le gâteau était trop bon.                                       &  \\
                                        &                                                                                  & \textit{because the cake was too good.}                                                           &  \\
de                                      & Die Gäste versteckten sich hinter dem Sofa und hielten den Kuchen, weil  & \cellcolor[HTML]{FFFFFF}weil sie sich nicht sicher waren, ob sie ihn wirklich essen würden.       &  \\
                                        &                                                                                  & \textit{unsure if they were actually going to eat it.}                                            &  \\
mn                                      & \begin{russian}Зочид бялуу барьж буйдангийн ард нуугдав, учир нь\end{russian}                     & \cellcolor[HTML]{FFFFFF}\begin{russian}учир нь өөрөө барьж буйдангийн ард нуугддаг.\end{russian}                              &  \\
                                        &                                                                                  & \textit{because the cake itself hides behind the sofa.}                                           &  \\
tg                                      & \begin{telugu}అతిథులు కేక్ పట్టుకుని సోఫా వెనుక దాక్కున్నారు కాబట్టి\end{telugu}                   & \cellcolor[HTML]{FFFFFF}\begin{telugu}కాబట్టి వారికి కేక్ పట్టుకుని సోఫా వెనుక దాక్కున్నారు అని అర్థం అవుతుంది.\end{telugu}  &  \\
                                        &                                                                                  & \textit{so it means they are holding the cake and hiding behind the sofa.}                        &  \\
ru                                      &\begin{russian}Гости спрятались за диваном, держа торт, потому что\end{russian}                     & \cellcolor[HTML]{FFFFFF}\begin{russian}потому что не хотели, чтобы их увидели.\end{russian}                                   &  \\
                                        &                                                                                  & \textit{because they didn't want to be seen.}                                                  & 

\\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Prompt examples for exploring multilingual NLI capabilities of mGPT on the COPA dataset~\cite{roemmele2011choice}. mGPT$_\text{1.3B}$ with pure sampling is used. The correct answer is \textit{``because this was a surprise party''}.}
\label{tab:nli}
\end{table*}

